Attack-aware Security Function Chain Reordering

Attack-awareness recognizes self-awareness for security systems regarding the occurring attacks. More frequent and intense attacks on cloud and network infrastructures are pushing security systems to the limit. With the end of Moore's Law, merely scaling against these attacks is no longer economically justified. Previous works have already dealt with the adoption of Software-defined Networking and Network Function Virtualization in security systems and used both approaches to optimize performance by the intelligent placement of security functions. However, these works have not yet considered the sequence in which traffic passes through these functions. In this work, we make a case for the need to take this ordering into account by showing its impact. We then propose a reordering framework and analyze what aspects are necessary for modeling security service function chains and making decisions regarding the order based on those models. We show the impact of the order and validate our framework in an evaluation environment. The effect can extend to multiple orders of magnitude, and the framework's evaluation proves the feasibility of our concept.

==> data/05_dynamic-reordering/modeling/single-functions_model_traffic.tex <==
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width = 35pt,
    enlargelimits=0.15,
    ylabel={Bandwidth Share in \%},
    symbolic x coords={1,2,3,4,5},
    xtick=data,
    xlabel={Traffic Class},
    %nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {(1,30) (2,10) (3,25) (4,20) (5,15)};
\end{axis}
\end{tikzpicture}
\vspace{3pt}

\centering
\begin{tikzpicture}
%\draw[blue!30] (0,0) grid[step=1] + (8,-5);
    \node[draw, single arrow,
          minimum height=9.5mm, minimum width=8mm,
          single arrow head extend=2mm,
          anchor=west, rotate=-90, fill = black] at (2,0) {};
    \node[draw,text width=5cm, align=center] at (2,-1.6) {Security Function \\ Defending Against Class 4};
    \node[draw, single arrow,
          minimum height=9.5mm, minimum width=8mm,
          single arrow head extend=2mm,
          anchor=west, rotate=-90, fill = black] at (2,-2.25) {};
\end{tikzpicture}
\vspace{3pt}

\begin{tikzpicture}
\begin{axis}[
    ybar,
    ymin = 0,
    bar width = 35pt,
    enlarge x limits=0.15,
    ylabel={Bandwidth Share in \%},
    symbolic x coords={1,2,3,4,5},
    xtick=data,
    xlabel={Traffic Class},
    %nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {(1,37.5) (2,12.5) (3,31.25) (5,18.75)};
\end{axis}
\end{tikzpicture}

==> images/architecture_fcc_reorder.tex <==
\begin{sequencediagram}
    \newthread{fcc}{FCC}{}
    \newinst[3]{sdn}{SDN}{}
    \newinst[1.5]{ovs}{Switch}{}
    \begin{callself}{fcc}{validate configuration}{}
    \end{callself}
    \begin{callself}{fcc}{start main thread}{}
    \end{callself}
    \begin{sdblock}{loop}{[Main Thread]}
    \postlevel
    \begin{call}{fcc}{\shortstack{New routing \\ configuration}}{sdn}{response}
        \begin{callself}{sdn}{generate flows}{}
        \end{callself}
        \begin{call}{sdn}{send flows}{ovs}{response}
            \begin{callself}{ovs}{apply flows}{}
            \end{callself}
        \end{call}
    \end{call}
    \postlevel
    \begin{callself}{fcc}{\shortstack{update current configuration \\ and reset attack list}}{}
    \end{callself}
    \end{sdblock}
\end{sequencediagram}

==> images/architecture_wrapper_keep-alive-loop.tex <==
\begin{sequencediagram}
    \newthread{wrapper}{Wrapper}{}
    \newinst[3]{fcc}{FCC}{}
    \begin{sdblock}{loop}{[Keep-alive Thread]}
        \begin{call}{wrapper}{send keep-alive}{fcc}{send new token}
            \begin{callself}{fcc}{validate}{}
            \end{callself}
        \end{call}
    \end{sdblock}
\end{sequencediagram}

==> images/architecture_wrapper_main-loop.tex <==
\begin{sequencediagram}
    \newthread{wrapper}{Wrapper}{}
    \newinst[3]{fcc}{FCC}{}
    \begin{sdblock}{loop}{[Main Thread]}
        \begin{callself}{wrapper}{validate attack report}{}
        \end{callself}
        \begin{call}{wrapper}{alert}{fcc}{response}
            \begin{callself}{fcc}{update attack list}{}
            \end{callself}
        \end{call}
    \end{sdblock}
\end{sequencediagram}

==> images/architecture_wrapper_start-stop.tex <==
\tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    transform shape,
    % set scale factor
    scale=1
  }
}

\begin{sequencediagram}
    \newthread{wrapper}{Wrapper}{}
    \newinst[3]{fcc}{FCC}{}
    \begin{callself}{wrapper}{validate configuration}{}
    \end{callself}
    \begin{call}{wrapper}{register}{fcc}{send token and ID}
        \begin{sdblock}{alt}{New Security Function}
            \begin{callself}{fcc}{add security function}{}
            \end{callself}
        \end{sdblock}
    \end{call}
    \postlevel
    \begin{callself}{wrapper}{start keep-alive thread}{}
    \end{callself}
    \begin{sdblock}{opt}{[Shutdown]}
        \begin{callself}{wrapper}{stop keep-alive thread}{}
        \end{callself}
        \begin{call}{wrapper}{delete}{fcc}{response}
            \begin{callself}{fcc}{remove security function}{}
            \end{callself}
        \end{call}
    \end{sdblock}
\end{sequencediagram}

==> sections/91_acknowledgement.tex <==
\section*{Publication of Software and Experiment Data}

We will publish all developed software, configuration files and experiment results, as well as a virtual Vagrant environment simulating our evaluation environment on GitHub upon acceptance.

\section*{Acknowledgment}

This work was co-funded by the German Research Foundation (DFG) under grant No. (KO 3445/16-1).
